ICE-SEARCH: A Language Model-Driven Feature Selection Approach

This study unveils the In-Context Evolutionary Search (ICE-SEARCH) method, which is among the first works that melds large language models (LLMs) with evolutionary algorithms for feature selection (FS) tasks and demonstrates its effectiveness in Medical Predictive Analytics (MPA) applications. ICE-SEARCH harnesses the crossover and mutation capabilities inherent in LLMs within an evolutionary framework, significantly improving FS through the model's comprehensive world knowledge and its adaptability to a variety of roles. Our evaluation of this methodology spans three crucial MPA tasks: stroke, cardiovascular disease, and diabetes, where ICE-SEARCH outperforms traditional FS methods in pinpointing essential features for medical applications. ICE-SEARCH achieves State-of-the-Art (SOTA) performance in stroke prediction and diabetes prediction; the Decision-Randomized ICE-SEARCH ranks as SOTA in cardiovascular disease prediction. The study emphasizes the critical role of incorporating domain-specific insights, illustrating ICE-SEARCH's robustness, generalizability, and convergence. This opens avenues for further research into comprehensive and intricate FS landscapes, marking a significant stride in the application of artificial intelligence in medical predictive analytics.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section/introduction_old.tex <==
\section{Introduction}  

The proposed \textbf{In-Context Evolutionary Search (ICE-SEARCH)} method is the first work that melds large language models (LLMs) with evolutionary algorithms for feature selection (FS) tasks and demonstrates its effectiveness in Medical Predictive Analytics (MPA) applications.

The core value of MPA resides in its ability to analyze the extensive datasets prevalent in the healthcare industry. This analytical power supports more informed clinical decision-making, enhances patient care quality, and facilitates more efficient allocation of healthcare resources. (\cite{lamba2021predictive}).

% 讨论一下FS的重要性
% 讨论一下FS的难点
% 引入EC-FS

% FS's application in MPA, widely adopted
However, this data's sheer volume and complexity pose significant challenges in converting it into actionable insights (\cite{Malik2016DataMA}). In this context, the feature selection (FS) process becomes critically important as it facilitates a more efficient analysis by identifying the most pertinent subset of features within high-dimensional datasets (\cite{massive_data}). 
For example, FS proves invaluable in stroke prediction, where data is extensive and varied as they are crucial for identifying key predictors among a large number of stroke risk factors (\cite{fs_stroke_1,fs_stroke2,fs_stroke3}). This approach can reveal insights into disease mechanisms, thereby enhancing medical research and improving patient care strategies (\cite{FSinMED}). 
Furthermore, evolutionary computation(EC)-based approaches have also proven to be an effective solution for feature selection given their global search ability(~\cite{EC4FS_survey}). 

Building data processing pipelines and machine learning models on large-dimension datasets faces significant challenges, primarily due to its expansive search space and the curse of dimensionality \cite{FS_eval_application}. As a data pre-processing technique, FS provides efficient and effective data preparation for data mining and machine learning problems (\cite{Li_2017}). This procedure can lower recognition costs by reducing necessary features and improving classification accuracy due to finite sample size effects (\cite{FS_eval_application}).

% These challenges include reduced generalizability, redundancy in complex problem scenarios, difficulties in managing high-dimensional data, a limited understanding of underlying data structures, and the requirement to assume data distributions that may not be valid.

On the other hand, the utility of Large Language Models (LLMs) has significantly evolved, extending far beyond traditional text analysis (\cite{zhao2023survey}). This evolution positions LLMs as critical instruments in specialized fields. The adaptability and advanced capabilities of these models are demonstrated by their leading-edge performance in various sectors, including medical diagnostics(~\cite{medpalm}), financial analysis(~\cite{bloombergGPT}), data preprocessing(~\cite{LLM4DataPrepro}), code generation(~\cite{codeLLaMA}), etc. This broad applicability underscores the potential of LLMs to revolutionize how we approach complex datasets and extract and interpret their most meaningful insights.
% 太长，空
% to FS in medical?
% evo method is a possible soln for FS

Furthermore, various research has shown the great potential of LLM to serve as a cross-over operator in evolutionary algorithms. As suggested by previous work (~\cite{chen2023evoprompting}), semantic knowledge encoded in the LLM allows for access to a considerable amount of \textbf{cross-domain knowledge} that would not be available in evolutionary algorithms, \textbf{greater diversity} of the outputs, and \textbf{reduces the amount of manual design and human bias} involved in the evolutionary algorithm, thereby powering evolutionary neuro-architecture search. Given the success of EC-based FS approaches, we posit that LLMs can effectively contribute to FS in various applications.

% MPA -> FS search space -> evo method -> LLM
% cite <<in context learning>>

% propose icesearch to solve problem ABCD
Hence, we introduce ICE-SEARCH, an FS methodology that integrates the in-context learning capabilities of language models (~\cite{ICL_Survey}) with an evolutionary algorithmic framework. Our method involves engaging the LLM in diverse roles, asking it to identify crucial features for a specific downstream task, and providing the LLM with feedback on the performance of both effective and ineffective feature sets, measured in terms of training and validation accuracies of 10-fold cross-validation(CV). We also discover that during evolutionary in-context training, there is an enhancement in the model's ability to uncover a set of high-quality feature combinations. %When submitting this manuscript, our research appears to be the first to explore the potential of LLMs in this context.
% 合起来下面两段
To demonstrate the efficacy of our approach, we analyze ICE-SEARCH's performance on three critical tasks- stroke prediction, cardiovascular disease prediction, and diabetes prediction- using three increasingly complex datasets. 
% Each of these diseases is among the leading causes of morbidity and mortality worldwide, carrying substantial risks of severe health complications, long-term disability, and death. 
We demonstrate that ICE-SEARCH consistently outperforms the existing FS methods in all three tasks. Interestingly, we perform a grid search of all possible feature combinations on Stroke and cardiovascular datasets. ICE-SEARCH is able to recover the best feature combination on the validation set. Additionally, our empirical studies show that ICE-SEARCH is robust against poor population initialization and fast convergence speed. 

%For example, according to the World Health Organization (WHO), ischemic heart disease is the top cause of death worldwide, accounting for 16\% of the world's total deaths. Stroke is the second leading cause of death and is responsible for approximately 11\% of total deaths (\cite{WHO_causeofdeath}). Additionally, diabetes has seen a substantial increase in mortality, now ranking as the 9th leading cause of death globally. (\cite{WHO_causeofdeath}).These diseases do not only lead to mortality but also cause long-term disability, which can profoundly affect the quality of life (\cite{WHO_mortalityhealthestimates}).



We summarize our contributions below:

\begin{enumerate}
    \setlength\itemsep{0.05em}
    \item Problem of FS in MPA or EC-FS, how ice search solves these issues.
    \item ICE-SEARCH is the first work to apply an LLM to iteratively search for valuable feature sets through role-playing and improve its in-context prompting examples without fine-tuning. 
    \item By integrating an evolutionary algorithm with LLM's in-context learning capability, ICE-SEARCH achieves SOTA performance in feature selection. Our experiments on three widely adopted MPA tasks demonstrate its effectiveness and robustness. 
    % \item The value of ICE-SEARCH lies in its ability to empower end-users with cross-domain expertise encoded in an LLM fine-tuned with domain-specific knowledge. 
    % ICE-SEARCH can be adapted to perform FS in areas like genetic analysis that commonly have thousands or even millions of features.
    % long-context ability
\end{enumerate} 




==> section/related_works_old.tex <==
\section{Related Work}
\label{sec:related_work}

% \textbf{Feature Selection: }
% FS presents itself as a difficult task mainly due to two challenges: (i) its vast search space, where the total possible solutions are $2^{n}$ for a dataset with n features, leading to exponential growth in computing expenses, and  (ii) the sub-optimal convergence caused by stagnations in local optima. Most of the techniques applied, such as heuristic search and random search, suffer from poor generalizability of evaluation criteria, redundant feature subsets when applied to complex problems~\cite{7339682}, huge search space for high-dimensional data whose efficiency deteriorates quickly or computationally infeasible~\cite{miao2016survey,li2017feature}, limited knowledge of the underlying data strucutre~\cite{li2017feature}, or imposing case-specific assumption(s) about the probability of the distribution of the data~\cite{miao2016survey}. Despite that evolutionary computation(EC) methods have shown promises~\cite{7339682}, flexible evaluation measures according to specific feature representations and search mechanisms that incorporate worldly knowledge across multiple disciplines are still in need for their optimal performance~\cite{li2017feature}. Feature selection algorithms that are scalable, robust against dataset quality, and efficient are preferred~\cite {doquet2020agnostic, li2017feature}.

% 行文逻辑：
% 1） FS是干啥的
% 2） FS问题的难点（cite OptFS）
% 3） EVO-FS的介绍
% 3.5） EVO-FS的缺点（cite survey），如果加，必须和4对应
% 4） 我们比一般的EVO-FS好在哪里（一句话）




\textbf{Feature Selection and its Evolutionary Solutions: }
Feature Selection (FS) is a critical dimensionality reduction technique used in data mining and machine learning to address the curse of dimensionality by selecting a relevant subset of features for model construction(~\cite{zebari2020comprehensive}), thereby preserving the original meanings of these features (~\cite{chandrashekar2014survey}). Its primary goal is to mitigate the impact of noise or irrelevant features in datasets, ensuring the accuracy and efficiency of predictions in subsequent models (~\cite{zebari2020comprehensive}). In practice, FS presents itself as a difficult task mainly due to its vast search space, where the total possible solutions are $2^{n}$ for a dataset with n features, leading to exponential growth in computing expenses(~\cite{OptFS}). Most of the techniques applied suffer from: (i) poor generalizability of evaluation criteria(~\cite{chandrashekar2014survey}), (ii) redundant feature subsets when applied to complex problems where partial correlations among the $2^{n}$ feature subsets complicate the determination of feature relevancy or redundancy(~\cite{7339682},~\cite{tuv2009feature}), (iii) huge search space for high-dimensional data whose efficiency deteriorates quickly or computationally infeasible(~\cite{miao2016survey,li2017feature}), (iv) limited knowledge of the underlying data structure(~\cite{li2017feature}), or (v) imposing case-specific assumption(s) about the probability of the distribution of the data(~\cite{miao2016survey}). Feature selection algorithms that are scalable, robust against dataset quality, and efficient are preferred(~\cite {doquet2020agnostic, li2017feature}).

As discussed in the survey(~\cite{FS_survey}), various ML and statistical FS algorithms have been proposed to tackle the task. In particular, as suggested by(~\cite{EC4FS_survey}), evolutionary computation (EC)-based approaches have recently proven effective in many scenarios. Specifically, EC methods for feature selection have been applied in scenarios including \textit{genetic algorithm}(~\cite{holland1992adaptation}), \textit{particle swarm optimization}(~\cite{wang2018particle}), \textit{genetic programming}(~\cite{muni2006genetic}), and \textit{correlation-based filter measures}(~\cite{hall1999correlation}). 

Apart from the prospect of evolutionary algorithms for FS, it points out several issues and challenges that need to be addressed: \textit{scalability}, \textit{computation cost}, \textit{search mechanisms}, \textit{stability}, etc. Specifically, the FS algorithms need to (1) have the capacity to process thousands or even millions of features, (2) have an efficient search strategy and a fast evaluation measure, (3) explore the whole search space and exploit the local regions if needed, and (4) be stable when using different starting points. 

Despite that EC methods have shown promise(~\cite{7339682}), they are not without limitations, often struggling with scalability and optimization efficiency in extremely high-dimensional spaces (~\cite{li2017feature}). Our approach surpasses conventional EC by integrating EC optimization techniques and pre-trained domain knowledge, significantly enhancing the accuracy and computational efficiency.


% \textbf{Evolutionary Algorithms for Feature Selection: }
% Due to the vast search space, finding an optimal feature subset remains a challenging task. As discussed in the survey written by~\cite{FS_survey}, various ML and statistical FS algorithms have been proposed to tackle the task. In particular, as suggested by~\cite{EC4FS_survey}, EC-based approaches have recently proven effective in many scenarios. Specifically, EC methods for feature selection have been applied in scenarios including \textit{genetic algorithm}~\cite{holland1992adaptation}, \textit{particle swarm optimization}~\cite{wang2018particle}, \textit{genetic programming}~\cite{muni2006genetic}, and \textit{correlation-based filter measures}~\cite{hall1999correlation}. Apart from the prospect of evolutionary algorithms for FS, it points out several issues and challenges that need to be addressed: \textit{scalability}, \textit{computation cost}, \textit{search mechanisms}, \textit{stability}, etc. Specifically, the FS algorithms need to: (1) have the capacity to process thousands or even millions of features, (2) have an efficient search strategy and a fast evaluation measure, (3) explore the whole search space and exploit the local regions if needed, and (4) be stable when using different starting points.

% \textbf{LLM for Feature Engineering:}  
% Feature engineering is closely related to feature selection, the former focuses on constructing new features from the original feature pool while the latter aims to identify and remove redundant and informative features. The article by~\cite{LLM4FE} introduces \textit{Context-Aware Automated Feature Engineering} (\textsc{CAAFE}), a method leveraging LLMs for automated feature engineering in tabular datasets. \textsc{CAAFE} uses LLMs to iteratively generate both the Python codes for creating new semantically meaningful features and explanations for their utility. The method improved performance on 11 out of 14 datasets, demonstrating its effectiveness over traditional methods. Similarly, CAAFE also combines the domain knowledge encapsulated in LLMs with classical machine learning algorithms, offering a novel approach to integrating domain knowledge into automated machine learning processes.

% Prompt is important for exploring LLM capability
% ex. cot tot, role-play, take a deep breath, 
% Evolutionary prompting: logic, benefit
% our method's difference
\textbf{Prompting and Evolutionary Prompting: }
Prompting is a technique employed to give LLMs leverage to address specialized tasks more efficiently. Various state-of-the-art prompting techniques, such as few-shot prompting (\cite{Brown2020LanguageMA}), Chain-of-Thought(COT) (\cite{Wei2022ChainOT}), Tree-of-Thought(TOT) (\cite{Yao2023TreeOT}), and Graph-of-Thought(GOT) (\cite{Besta2023GraphOT}) have been proven effective in tackling various tasks such as cross-lingual multi-step reasoning \cite{Ranaldi2023EmpoweringMR}, vision-language pre-training \cite{Mu2023EmbodiedGPTVP}, and Big-Bench \cite{Suzgun2022ChallengingBT}, which encompasses 204 tasks from diverse topics(ex. linguistics, childhood development, math) that are believed to be beyond the capabilities of current language models.
However, the performance of LLMs varies depending upon the selection of the prompt (~\cite{liu2023pre}), and that leads to automatic prompt optimizations, such as continuous prompt tuning (~\cite{li2021prefix}) and differentiable prompts(~\cite{zhang2021differentiable}). 
% Relationship between general icl, evolutionary prompting, and our works
In contrast, the high variance in prompt effectiveness for downstream tasks has led to the development of prompt engineering (~\cite{zhou2022large}), prompt revision (~\cite{guo2023learning}), and prompt editing (~\cite{zhang2022tempera}) methods that focus on the exploration or exploitation of candidate prompts to select the most optimal one(s). 

% which may encounter challenges when applied to generation tasks,
To address the constraints of prompts designed for predefined answers and to mitigate the risk of encountering local optima, many have explored evolutionary prompting optimization techniques (~\cite{Yang2023LargeLM, Meyerson2023LanguageMC, guo2023connecting,chen2023evoprompting}). They offer the advantages of not relying on predefined parameters or gradients while simultaneously maintaining a balance between exploration and exploitation. 
Such paradigms of evolutionary prompting inspired ICE-Search, which adapts and evolves in the search for optimal prompts to identify critical features for downstream tasks. 
Similar to evolutionary prompting, ICE-Search showcases novel ways of leveraging language models while offering flexibility and adaptability to diverse metrics and tasks.

% 放到最后一节
\textbf{Medical Predictive Analysis: }
Medical Predictive Analytics (MPA) represents a critical and specialized sector within health informatics dedicated to sophisticated medical data examination. MPA leverages advanced statistical algorithms and machine learning methodologies to forecast upcoming trends in healthcare outcomes, including patient admission rates, pharmaceutical advancements, and strategies for disease management (\cite{van2019predictive}). For example, previous works have focused on leveraging various algorithms to facilitate predictive data mining for medical diagnosis(~\cite{soni2011predictive}), disease prediction(~\cite{Usama2019SelfattentionBR}), robotic surgery(~\cite{Oniani2020ArtificialIF}), use of disease diagnosis systems for Electronic Medical Records(~\cite{Latif2020ImplementationAU}), as well as analysis and prediction of outpatient visits(~\cite{Jin2019PredictiveAI}).
